FOCAL: A Cost-Aware Video Dataset for Active Learning

In this paper, we introduce the FOCAL (Ford-OLIVES Collaboration on Active Learning) dataset which enables the study of the impact of annotation-cost within a video active learning setting. Annotation-cost refers to the time it takes an annotator to label and quality-assure a given video sequence. A practical motivation for active learning research is to minimize annotation-cost by selectively labeling informative samples that will maximize performance within a given budget constraint. However, previous work in video active learning lacks real-time annotation labels for accurately assessing cost minimization and instead operates under the assumption that annotation-cost scales linearly with the amount of data to annotate. This assumption does not take into account a variety of real-world confounding factors that contribute to a nonlinear cost such as the effect of an assistive labeling tool and the variety of interactions within a scene such as occluded objects, weather, and motion of objects. FOCAL addresses this discrepancy by providing real annotation-cost labels for 126 video sequences across 69 unique city scenes with a variety of weather, lighting, and seasonal conditions. We also introduce a set of conformal active learning algorithms that take advantage of the sequential structure of video data in order to achieve a better trade-off between annotation-cost and performance while also reducing floating point operations (FLOPS) overhead by at least 77.67%. We show how these approaches better reflect how annotations on videos are done in practice through a sequence selection framework. We further demonstrate the advantage of these approaches by introducing two performance-cost metrics and show that the best conformal active learning method is cheaper than the best traditional active learning method by 113 hours.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> Sections/Abstract.tex <==
We introduce \texttt{FOCAL} (Ford-OLIVES Collaboration on Active Learning) - the first publicly available video dataset that has annotation cost for training active learning models. While several public video datasets are available to benchmark active learning performance, they lack real time annotation labels for accurately assessing cost minimization. \texttt{FOCAL} has real time cost annotations for 126 video sequences across 69 unique scenes in an infrastructure setting from a variety of weather, lighting, and seasonal conditions. This creates opportunity for richer analysis to better understand annotation cost statistics in videos and design algorithms based on annotation workflows. In video object detection, annotation workflows utilize the sequential nature of motion to label objects across frames. We imbue this annotation workflow in active learning by proposing a suite of conformal sampling algorithms based on video statistics that query sequences rather than frames. Conformal sampling, unlike existing inferential sampling, refers to sampling strategies that do not need inferential distribution of the unlabeled pool to rank sample importance at the end of every round. This reduces the overall floating point operations overhead of conformal sampling algorithms by at least $77.67 \%$. We develop two performance-cost benchmarking metrics and show that the best conformal active learning method is cheaper than the best inferential method by 113 hours. 



% We propose the \texttt{FOCAL} (expansion retracted to maintain anonymity) dataset - the first annotation-cost-centered video sequence dataset for active learning applications. While current open-source datasets are effective in benchmarking active learning approaches, they are not originally intended for active learning research and lack crucial characteristics for effective evaluation of different algorithms. Specifically, they lack cost information for annotating data samples. For this reason, current approaches naively assume that annotation cost scales with the annotated training pool size linearly. In practice, this assumption is rarely correct. \texttt{FOCAL} represents the first dataset that allows researchers to benchmark active learning algorithms in a cost-centered manner that is not dependent on the amount of annotated samples. In addition to the dataset, we provide practically relevant benchmarks in sequential, as well as singular active learning settings. We find that existing algorithms largely neglect annotation cost information and performance scales similarly to random sampling in terms of temporal annotation cost. To the best of our knowledge, \texttt{FOCAL} is the first dataset to provide a sequential, cost-centered environment for active learning algorithms. It consists of a plethora of real-world scenarios that include
% 142 sequences, 109, 000 frames, and 79 unique scenes across
% a variety of weather, lighting, and seasonal conditions. We benchmark performance across $5$ query strategies for the task of 2D object detection and  analyze their behavior in terms of annotation-time cost and test set performance.

==> Sections/Conclusion.tex <==
\section{Conclusion}
In this paper, we introduced \texttt{FOCAL} - the first public cost-aware video active learning dataset for object detection. In addition to \texttt{FOCAL} being used as a benchmark to cost-conscious video active learning, it will also serve to benchmark object detection. With the goal of active learning in mind, we conduct a detailed cost analysis to understand the factors that induce cost during the human annotation of video sequences. We then exploit these factors to design conformal active learning sampling algorithms. With \texttt{FOCAL} having prospective real time annotation labels, it paves an avenue for accurate, practical, cost-oriented video active learning approaches. It also allows in depth performance-cost analysis using mAP versus cost curves along with CAR and PAR metrics. We see \texttt{FOCAL} as a first step of many in bringing video active learning approaches closer to practical deployment.


==> Sections/CostAnalysis.tex <==
\section{Cost Analysis of FOCAL Dataset} 
\label{sec:costAnalysis}
\vspace{-2mm}
\paragraph{Dataset Curation}
The locations of these video sequences are selected to obtain a wide range of interactions that are at the intersection of infrastructure-assisted autonomy and autonomous vehicle communities. The locations include urban intersections, shopping zones, college campuses, etc. Additionally, \texttt{FOCAL} has a diverse range of environmental (snow, rain, and sun) and lighting conditions (morning, noon, and evening) as well as a wide variety of scenes as shown in Figure \ref{fig: space_temp_diversity}. Furthermore, the collection of data from January to August enables the dataset to have variation in terms of seasons. The resulting dataset contains 103,518 frames across 126 individual sequences and 69 unique scenes. Every sequence is labeled by annotators for 2D bounding boxes, tracking identities, and category specific object attributes such as if the doors of a car are open or not. Objects are labeled to be one of 23 possible classes. In our experiments, we have consolidated these 23 classes into 4 super classes: Pedestrian, Bicycle, Car and Cart. During the annotation process for each sequence, time information regarding the usage of the labeling platform by each annotator is tracked. The annotation cost label of a sequence is the cumulative time of all users that performed any labeling or quality assurance on the sequence. Additional details ad statistics regarding dataset collection, object labels, metadata labels, scene and object diversity can be found in Appendix \ref{app:stats}. The rest of Section~\ref{sec:costAnalysis} is dedicated to understanding the factors that contribute to the notion of annotation cost.
\vspace{-2mm}
\paragraph{Number of Bounding Boxes} It makes intuitive sense that sequences with a large number of bounding box annotations take longer to annotate and thus have a higher cost. This is shown in Figure \ref{fig:cost_analysis}(a). However, in an active learning framework, one does not have access to the true number of bounding box annotations when making queries. We use optical flow maps to estimate the box count, as described in Section~\ref{sec:Methodology}. The relationship between estimated box count and cost is shown in Figure \ref{fig:est_queries}(b) in the supplementary material.
\begin{figure}[t!]
\centering
\includegraphics[width = \columnwidth]{Fig/cost_analysis/cost_analysis_variables.png}
\caption{The relationship between cost and: (a) Number of boxes. (b) Occlusion severity.}
\label{fig:cost_analysis}
\end{figure}
\vspace{-2mm}
\paragraph{Occlusion Severity} The labels for objects that are partially or fully hidden by other objects in a sequence are available in \texttt{FOCAL}. Figure \ref{fig:cost_analysis}(b) shows that the annotators take more time to label occluded objects thus increasing cost. However, similar to bounding box count, access to occlusion status is unavailable at query time and query strategies that use occlusion as a measure must estimate the severity. 
\vspace{-2mm}
\paragraph{Motion} With sequential data, annotation is performed in blocks. When there is motion between frames it is intuitive to assume it takes more time (higher cost) to create bounding box annotations. This is because the annotator needs to locate the new position of the object each time it moves. On the other hand, bounding box annotations for static objects are copied across multiple frames at zero cost \cite{yuen2009labelme}. However, this linear relationship between motion and annotation cost does not always hold. This occurs when the high motion object was not an object being annotated. For example, a tree constantly blowing from strong winds has high motion but trees were not an object being annotated for this dataset. The relationship between estimated motion via optical flow and annotation cost is shown in Figure \ref{fig:est_queries}(a) in the supplementary material.
\vspace{-2mm}
\paragraph{Sequence Length} This is the number of frames in each video sequence. Although it seems intuitive that the length of a sequence is proportional to the annotation cost, this was not the case in \texttt{FOCAL}. A long sequence may or may not contain many relevant objects to be annotated and the same is true for a short sequence. As such, cost is independent of the length of a sequence, as visualized in Figure \ref{fig:intro-cost-perf}(b).

% \paragraph{Object Density} Object density is defined as the $\frac{number \ of \ objects}{sequence \ length}$. Therefore, without knowing the true number of objects, object density is also unknown at query time. Since the length of a sequence is independent of cost, scaling the number of objects by this constant reveals no additional information about cost. 


% \paragraph{Change of Object Quantity}
% We consider the temporal first-order statistics of the accumulative object quantity of each sequence as a factor of annotation cost. Specifically, we calculate this quantity as the change of object quantity between a certain fixed number of frames. A higher number of mobile objects moving in and out of the frame can result in higher annotation costs due to more efforts in accurately tracking these objects. 

% \paragraph{Velocity of Objects}
% Annotation costs can be higher when there are objects moving faster. We calculate the accumulative velocity in normalized pixels of objects to quantify the magnitude of the variance of motion. 

% The following part does NOT add values... check Fig/cost_analysis/Var_ObjectDensity_vs_Cost.png, there is no trend.
% \paragraph{Variation of Object Density}
% Statistical dispersion of object density can also cause varying cost values. It is likely to take more annotation efforts to track more mobile objects that move in and out of the field of view. The standard deviation of object density is calculated as $std(\frac{number \ of \ objects}{sequence \ length})$ to quantify such variation. 

% \begin{figure}[h!]
% \centering
% \includegraphics[width = \columnwidth]{Fig/cost_analysis/VelocityofObjects_vs_Cost.png}
% \caption{Velocity of Objects.}
% % \label{fig:cost_analysis}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \includegraphics[width = \columnwidth]{Fig/cost_analysis/Var_ObjectDensity_vs_Cost.png}
% \caption{Variation of Object Density.}
% % \label{fig:cost_analysis}
% \end{figure}

==> Sections/Dataset.tex <==

\section{FOCAL Dataset}
% Chen: this is fig 3 that needs to be in the appendix
% \begin{figure}[h!]
% \centering
% \includegraphics[width = \columnwidth]{Fig/map.JPG}

% \caption{The \texttt{FOCAL} data was collected at various locations across southeastern Michigan (mainly in Ann Arbor and Detroit). Stars indicate  examples of where data acquisition took place with the Smart City Van. \vspace{-.3cm}}

% \label{fig: map}
% \end{figure}
\paragraph{Dataset Curation}
The locations of these video sequences were selected based on the intent to obtain a wide range of interactions that are at the intersection of infrastructure-assisted autonomy and autonomous vehicle communities. The locations include urban intersections, shopping zones, college campuses, etc. Additionally, we want to have a diverse range of environmental and lighting conditions such that sufficient variation exists in regards to real-world conditions. This can be understood through Figure \ref{fig: space_temp_diversity} where we observe the wide variety of scenes, weather conditions (snow, rain, and sun), and lighting conditions (morning, noon, and evening) that exist within the \texttt{FOCAL} dataset. Furthermore, the collection of data from January to August enables the dataset to have variation in terms of seasons. The resulting dataset contains 103,518 frames across 126 individual sequences and 69 unique scenes. Every sequence is labeled by annotators for 2D bounding boxes, tracking identities, and category specific object attributes such as if the doors of a car are open or not. Objects are labeled to be one of 23 possible classes but, for our experiments, have been consolidated into 4 super classes: Pedestrian, Bicycle, Car and Cart. During the annotation process for each sequence, time information regarding the usage of the labeling platform by each annotator is tracked. The annotation cost label of a sequence is the cumulative time of all users that performed any labeling or quality assurance on the sequence. Additional details about dataset curation, object labels, metadata labels, scene and object diversity can be found in Appendix \ref{app:stats}.

% Chen please put these in the appropriate sections of the supplementary material 
% \paragraph{Object Labels}
% All data taken from these mounted cameras is fed into a labeling platform. Image data is fed into a tool to anonymize the sequence for sensitive information, e.g., blurring the faces of people and the license plates of cars. Every sequence is then labeled by annotators for 2D/3D bounding box coordinates, tracking identities, and state labels for various agent interactions, such as whether a vehicle is parked or not. These annotations took place at a rate of 1 Hz. Objects are labeled to be one of 23 possible classes as shown by the left graph in Figure \ref{fig: class_cost_dist}.  In our active learning experiments, the 23 classes have been consolidated into 4 super classes: Pedestrian, Bicycle, Car and Cart. After annotations were completed for an individual sequence, the sequence is sent for review to a separate team who performs quality assurance for the curated annotations. This is done to minimize bias in annotations. 

% During the annotation process for each sequence, time information regarding the usage of the labeling platform by each annotator is tracked. The annotation cost label of a sequence is the cumulative time of all users that performed any labeling or quality assurance on the sequence. The cost for each sequence varies as shown by the right graph in Figure~\ref{fig: class_cost_dist}. Here we show a histogram of the time spent labeling in minutes compared to the number of sequences within the dataset. However, there is still some variation in annotation-cost time that indicates the \texttt{FOCAL} dataset has both hard and easy to label sequences. This is beneficial for distinguishing active learning strategies, i.e., an optimal strategy should select sequences with less time to annotate over others, while simultaneously optimizing for performance.

% \paragraph{Metadata} 
% Within the label file for each image, there is a variety of associated meta data specific to the type of object. For vehicles, this includes a label that is indicative of parking or not. For pedestrians, there are labels indicating whether the pedestrian is crossing the street or not. Finally, for every object there is an occlusion label. This label indicates whether the associated object is hidden behind another object, partially hidden, or fully visible within the current frame.

% \paragraph{Scene Diversity} To obtain training, test and validation sequences in non-overlapping scenes, we manually group all sequences into 69 unique scenes. These scenes contain diverse spatial structures (e.g., urban intersections and highways), and various weather and lighting conditions (e.g., sunny, cloudy, and rainy) as illustrated in Figure \ref{fig: scene_id}. The sequences were collected in a wide range of seasons from winter to summer. The ratio of each season is depicted in the \textcolor{blue}{supplementary material}. Overall, there are 10.30\%, 63.49\%, and 26.21\% sequences collected in the winter, spring, and summer, respectively. In summary, our scene selection encourages diverse data conditions to evaluate active learning algorithms. 

% \paragraph{Object Diversity} In addition to the scene diversity, object diversity is also present in the \texttt{FOCAL} dataset. As shown in the left graph in Figure \ref{fig: scene_id}, the overall semantic categories include various types of pedestrians, vehicles, static scene objects, etc. As shown in the supplementary material, the number of object instances varies across sequences due to the scene as mentioned above diversity. For instance, we observe that the sequences collected in the summer contain more objects with diverse activities compared to the sequences collected in the winter. 

% \begin{figure*}[t]
% \centering
% \includegraphics[scale = .65]{Fig/class_cost_dist_ICML.pdf}

% \caption{\texttt{FOCAL} dataset class distribution and variation of cost annotations. Left: Log-scaled class distribution. The y-axis shows the number of object instances for each class in the \texttt{FOCAL} dataset. Right: Variation of cost within frames in sequence. The variation is beneficial for distinguishing active learning algorithms to identify optimal strategies that simultaneously select sequences with less time to annotate and optimize for performance.\vspace{-.3cm}}

% \label{fig: class_cost_dist}
% \end{figure*}



==> Sections/Introduction.tex <==
\section{Introduction}

% Outline 
% traditional supervised Learning compared to AL
% The goal of AL (reduce cost, max performance) 
% Previous work assumes constant cost but this isnt true across all domains eg. text, video 
% Lots of research on text, very little on video 
% most works reduce cost by reducing samples. no investigating other cost contributors 
% Our contributions :
    % dataset
    % cost analysis 
    % benchmarks
    % cost-sensitive video queries 
    % answer questions: does min cost automatically max performance?

\label{sec:intro}
Supervised learning has been widely studied across multiple domains and it is no secret that these algorithms require thousands (even millions) of annotated data samples to maximize performance. Acquiring large volumes of annotated data is a tedious, time-consuming and costly task, particularly for sequential data domains like speech, text and video. Active learning frameworks are designed to counter this bottleneck as an experimental optimization problem. Its goal is to induce a model to achieve maximal performance at minimal cost \cite{settles2009active}. Here, achieving maximal performance at minimal cost implies selecting the most informative subset of samples that incur the least human annotation time to train a model. 

\begin{comment}
\begin{figure} [t!]
\centering
\includegraphics[width=\columnwidth]{Fig/intro_fig.png}
\caption{(a) Test set performance in terms of mean average precision (mAP) for singular (frame-wise) sampling in comparison to their sequential counterparts of three uncertainty methods: entropy, margin, and least confidence sampling \cite{settles2009active}. (b) The cost is independent of the number of frames in a video sequence.}\vspace{-5mm}
\label{fig:intro-cost-perf}
\end{figure} 
\end{comment}
However, it is to be noted that the majority of active learning research has not concerned itself with accurate cost accounting. In fact, existing datasets are not usually created for the purpose of active learning and lack real-time cost annotation labels. Rather, approximate cost is naively assumed to share a linear relationship with the number of samples in the dataset \cite{settles2008activecost, bloodgood2014bucking}. Therefore, several studies minimize cost by reducing the number of samples queried. For example, \cite{vondrick2011video} propose a video active learning algorithm that minimizes cost by selecting frames not having stationary objects or objects moving in isolation. However, this assumption of a linear relationship between cost and samples is not valid across all application domains, particularly video. We show this in Figure \ref{fig:intro-cost-perf}(b) where the relationship between cost and sequence length (number of frames in a video) shows that the cost is independent of the number of frames in a sequence. In fact, variation in cost results from multiple other factors. Consider that when labeling videos for object detection, annotators label sequential frames in blocks to allow for more efficient labeling \cite{yuen2009labelme}. In doing so, the bounding box labels of static objects can be copied in between frames at zero cost. Additionally, object motion, object density, occlusion severity, distance of objects from the sensor, weather and lighting conditions all influence whether certain sequences incur more time to annotate.

Within the active learning research cohort, most cost-conscious active learning literature is in the domain of natural language processing (NLP). However, considerably less attention has been given to video active learning because of a lack of video datasets with real cost information. This is detrimental to existing methods~\cite{vondrick2011video} as they treat video active learning as an extension of image-wise active learning. They sample the unlabeled pool for images irrespective of which video these images are derived from. However, this does not match the human annotation workflow where objects are labeled across a video. Even though these methods may lead to higher performance, this is in fact an overestimated performance when realistic settings are taken into consideration. In Figure~\ref{fig:intro-cost-perf}(a), we show this behavior empirically by analyzing popular active learning algorithms defined on single video frames, as well as their sequential implementation on video sequences. In the single setting, we treat videos as a collection of images. The active learning strategies are given the freedom to sample any images in a given round. In the sequential setting, an active learning algorithm can only sample sequences. We see that sequential implementations generally perform worse in terms of test set mean average precision (mAP) than their singular frame-wise counterparts indicating performance overestimation. Hence, there is a clear need for an active learning dataset dedicated to video-relevant practical scenarios with annotation cost as a central evaluation metric along with detection performance. 

In order to alleviate this need, we introduce the \texttt{FOCAL} video active learning dataset intentionally annotated in sequences and the annotation cost prospectively recorded in hours. We design algorithms that query video sequences rather than single frames to match the annotation workflow. In designing our query algorithms we show the efficacy of exploiting spatial and temporal statistics of videos to minimize cost while maximizing performance. Within the context of active learning we refer to these methods as \textit{conformal sampling}, inspired by \cite{angelopoulos2021gentle}. We use conformal sampling in a setting where we do not need inferential distribution of the unlabeled pool to rank the importance of samples. We also design two performance-cost benchmarking metrics to evaluate conformal and inferential video active learning algorithms. In summary, the contributions of this paper are as follows:
\vspace{-2mm}
\begin{itemize}
\item We introduce the first public video active learning dataset accompanied by detailed annotations and annotation time, that provides a rigorous basis for accurate quantitative evaluation of annotation cost reduction in active learning research. 
\item We conduct a detailed analysis of multiple factors that affect the annotation cost of video sequences. 
\item We provide a new benchmark for object detection and cost-conscious video active learning on \texttt{FOCAL}. 
\item We compare adaptions of traditional inferential sampling to conformal sampling on video sequences.
\item We introduce two new performance-cost metrics for validating the effectiveness of query strategies minimizing cost while maximizing performance.
\item The presence of video statistics allows us to front-load ranking of the unlabeled pool, thus reducing overhead cost by greater than 8 million GFLOPS.
\end{itemize}




==> Sections/Methodology.tex <==
\section{Experimental Setup}
\label{sec:Methodology}
\subsection{Object Detection} We benchmark \texttt{FOCAL} on $6$ architectures to establish how challenging it is for object detection using YOLOv3, YOLOv3-tiny \cite{redmon2018yolov3}, CenterNet \cite{duan2019centernet} and YOLOv5n, YOLOv5m, YOLOv5x \cite{Jocher_YOLOv5_by_Ultralytics_2020}. The training, test, and validation sets consist of $86, \ 27, \ 13$ sequences, respectively. The classes in the \texttt{FOCAL} are grouped into 4 superclasses, i.e.,  pedestrian, bicycle, car, and cart, for both training, validation and testing. Each architecture is trained for a total of $30$ epochs. In order to evaluate detection performance, we report mean average precision (mAP) at IOU thresholds $0.5$ (mAP@$50$), and mAP between $0.5$ and $0.95$ (mAP@$[50, 95]$). Additional details about experimental setup and data access can be found in Appendices \ref{app:link} and  \ref{app:setup}.

\subsection{Sequence Active Learning for Object Detection}
For active learning, all experiments were conducted using a YOLOv5n architecture. Within each active learning round, the model is trained for 10 epochs. After each epoch, the best model with respect to the validation set is saved to evaluate the test set for that round. This is repeated with three different random seeds and an average mAP was aggregated. 
\vspace{-2mm}
\paragraph{Inferential Sampling} In our experiments, we consider traditional active learning algorithms that need to compute posterior probabilities  to rank samples in the unlabeled pool as inferential approaches. We adapt these algorithms, defined on single frames, to entire video sequences. We evaluate the acquisition function on entire sequences of statistically dependent data in the form of $s_i = \{x_{i,1}, ..., x_{i,N}\}$. Here $x_{i,k}$ represent the individual statistically dependent data points and $N$ the sequence length. The acquisition function scores individual sequences by:

\begin{equation}
\label{eq:seq-al}
    S^* = \argmax_{s_1, ..., s_b \in S_{pool}} a(s_1, ..., s_b | g(f_w, s))
\end{equation}

where $g$ represents a summary function that combines the network output of entire data sequences, $S_{pool}$ the unlabeled data sequences. In our implementations (and \texttt{FOCAL} benchmarks), we reduce $g$ to be the arithmetic mean of the scores on each frame.

In our probabilistic sampling experiments, we start with two randomly chosen sequences and select one additional sequence in every round until the training pool has a total of 13 sequences. To perform active learning experiments for object detection, we adapt existing algorithms from classification to object detection settings. For entropy, which is based on softmax probabilities \cite{wang2014new}, we use the object probability of each YOLOv5 grid in the output prediction and derive a single acquisition function score for each grid. Each frame score is then reduced to averaging the grid scores within a single frame. Following this intuition, we evaluate the sequence score by averaging all frame scores within a sequence. For FALSE \cite{benkert2022false} and GauSS \cite{benkert2022gauss} we define the switching score as the difference between the predicted number of objects in between rounds for each frame and produce a sequence score by calculating the arithmetic mean across all frames. We sample the highest switching scores for FALSE while GauSS approximates the switching score distribution with a two component Gaussian mixture model and samples from the component with a higher switch mean. As a standard baseline we further perform random sampling where we randomly select the next batch of video sequences from the unlabeled pool.

\paragraph{Conformal Sampling} These sampling strategies are based on estimates of the factors that contribute to cost as discussed in Section \ref{sec:costAnalysis} with the goal of it being minimized. Inferential strategies are typically model dependent. However, conformal sampling does not require posterior probabilities from a trained model to select samples from the unlabeled pool. One advantage of conformal sampling is that it negates the need to begin active learning with random samples. Rather, each algorithm selects its initial samples according to its unique criteria. The following are a descriptions of the conformal sampling algorithms proposed in this study:

\begin{figure} [t!]
\centering
\includegraphics[width=0.85\columnwidth]{Fig/true-cost-vs-exp-cost.png}
\caption{We compare annotation cost, in hours, of all sampling algorithms to the theoretical upper and lower cost bounds of the \texttt{FOCAL} dataset. Shaded curves show the average cost and standard error for algorithms with stochastic cost.}
\label{fig:upper-lower-cost-bounds}
\end{figure} 

\begin{itemize}
\item Least Frame: A sequence length based approach that selects $k$ sequences with the shortest length $l(k)$.
\begin{equation}
\label{eq:least-frame}
    k^* = \argmin_{k} l(k)
\end{equation}
\item Most Frame: A sequence length based approach that selects $k$ sequences with the longest length $l(k)$. 
\begin{equation}
\label{eq:most-frame}
    k^* = \argmax_{k} l(k)
\end{equation}
\item Motion: A motion-based approach that uses optical flow \cite{fleet2006optical} as a metric to rank sequences according to its temporal information. Optical flow maps for each sequence are generated using a PWC-Net \cite{sun2018pwc} model trained on the KITTI 2015 dataset \cite{geiger2015kitti}. Motion scores, $\Sigma_{i = 0}^{N}m_i(k)$, are generated by summing the pixel values of each flow map within an sequence. Low motion sequences would have smaller pixel values in their flow maps and the opposite is true for high motion sequences.  $N$ is the number of frames in a sequence. 
    \begin{itemize}
        \item Min Motion: This selects $k$ sequences with the lowest motion scores
        \begin{equation}
        \label{eq:min-motion}
            k^* = \argmin_{k} \Sigma_{i = 0}^{N}m_i(k)
        \end{equation}
        \item Min Max Motion: This selects $k$ sequences having either the lowest or highest motion scores at alternating rounds $r$.

        \[ k^* = \begin{cases} 
              \argmin_{k} \Sigma_{i = 0}^{N}m_i(k) & r \in E \\
              \argmax_{k} \Sigma_{i = 0}^{N}m_i(k) & r \in O \\
           \end{cases}
        \] 
        $E$ and $O$ are the set of even and odd numbers respectively.
    \end{itemize}
\item Min Boxes: A sampling approach that uses the spatial distribution of pixels in optical flow maps to estimate the number of boxes $\Sigma_{i = 0}^{N}b_i(k)$ in a sequence. The spatial information is used to estimate the number of boxes in a sequence for $k$ sequences with the lowest estimated box counts to be selected.
        \begin{equation}
        \label{eq:min-boxes}
            k^* = \argmin_{k} \Sigma_{i = 0}^{N}b_i(k)
        \end{equation}
\end{itemize}

In Figure \ref{fig:upper-lower-cost-bounds}, we validate these conformal sampling strategies based on the insights gained from the cost analysis in Section \ref{sec:costAnalysis}. We show where annotation cost of each sampling method lies with respect to the theoretical bounds (dashed lines) of \texttt{FOCAL}. Theoretical upper and lower bounds were computed by selecting sequences in descending and ascending cost order, respectively, then summing cumulatively. For ease of visualization, we show the first seven active learning rounds. Using the estimates of motion in conformal sampling, the red and green curves are closer to the theoretical minimum (dashed light blue). Since cost is independent of sequence length, it is not surprising that least and most frame sampling (blue and orange curves) have cumulative costs closer to the upper bound (dashed dark blue). Inferential methods are associated with a stochastic annotation cost and the average and standard error of each is shown as a shaded curve.

\subsection{Performance-Cost Metrics}
Within the context of active learning, cost analysis is especially relevant when considered jointly with generalization performance. For instance, selecting low cost video sequences is less relevant when no additional detection performance gain is expected. For this purpose, we visualize changes in both via mAP versus cost plots. The x-axis represents the cost, in hours, of labeling the number of sequences in the training pool and the y-axis is the mAP the model achieves on the test set. Based on this, we develop two metrics to study performance-cost evaluation: cost appreciation rate (CAR) and performance appreciation rate (PAR). 
% Mathematical definitions of these can be found in Appendix \ref{app:setup} of the supplementary material.

\paragraph{Cost Appreciation Rate}
The cost appreciation rate is the area under the mAP vs cost curve at different cost budgets. CAR is defined as follows:

\begin{equation}
\label{eq:car}
    CAR = \int_{0}^{b} AP({c}) \,dc.
\end{equation}

where $b$ is the cost budget, $c$ is a cost value less than the budget, and AP({c}) is the corresponding mAP on the y-axis for cost value $c$. CAR plots shown in Section \ref{sec:results} answer the question, "With cost-focused budgets leading up to 200 hours maximum, which algorithm results in the highest performance at each budget?". Here, high CAR values indicate the better algorithm.

\paragraph{Performance Appreciation Rate}
Similar to CAR, the performance appreciations rate is the area under the mAP vs cost curve at different performance budgets. PAR is defined as follows:

\begin{equation}
\label{eq:car}
    PAR = \int_{0}^{b} AP({p}) \,dp.
\end{equation}

where $b$ is now the performance budget, $p$ is a performance value less than the budget, and $AP({p})$ is the corresponding cost on the x-axis for performance value $p$. PAR plots shown in Section \ref{sec:results} answer the question, "With budgets leading up to 0.6 mAP, which algorithm achieves the lowest cost at each budget?". Low PAR is indicative of the better algorithm.

\paragraph{Overhead Computation Cost}
There is an additional component that contributes to cost other than annotation time. This comes directly from the sampling algorithm and in this context, we call this an overhead cost. For inferential sampling techniques (except random), overhead cost is defined as the number of floating point operations per second (FLOPS) YOLOv5n executes to compute the posterior probabilities of the unlabeled pool for all active learning rounds. The overhead cost for Min Boxes, Min Motion and Min Max Motion conformal sampling is the FLOPS of PWC-Net to compute the optical flow maps for the available data before beginning active learning. Random, Least Frame and Most Frame sampling have zero overhead cost. We use the flopth library \cite{Wang2021} to calculate the FLOPS of YOLOv5n for inference on a single \texttt{FOCAL} frame and for a pair of frames on PWC-Net. 




==> Sections/RelatedWork.tex <==
\section{Related Works}
% ------ Outline --------
% Active learning
% Cost measurment
% Cost focused sampling
    %  NLP 
    % video 
% AL for text/video 

%In order to highlight the utility of the \texttt{FOCAL} dataset, an understanding of the gaps in active learning research is necessary. 
%In this section, we first present conventional active learning research, before discussing active learning studies that have more complex problem settings and require extensions to the traditional approaches.
\input{Tables/DatasetComparisons.tex}
\paragraph{Active Learning} Active learning is a widely researched area of machine learning \cite{settles2009active}. Traditional methods typically involve a model iteratively selecting samples for annotation from an unlabeled data pool until an annotation budget is reached. Approaches for how the samples are selected differ in their definition of information content for samples within the unlabeled data pool. As an example, several approaches define sample importance using softmax probabilities \cite{wang2014new, roth2006margin} where information content is related to the output logits of the network. Other works focus on constructing the core-set of the unlabeled data pool \cite{sener2017active, longtailcoreset}. Furthermore, there are several approaches that consider the combination of both data representation and generalization difficulty within their definition of information content \cite{ash2019deep, prabhushankar2022introspective, haussmann2020scalable}. In those studies, an ordering is established based on generalization difficulty and the representative component is introduced by sampling interactively from the ordering. \cite{batchbald} integrates both generalization difficulty and data representation by extending \cite{houlsby2011bayesian} to diverse batch acquisitions. Recent work \cite{benkert2022gauss} has defined sample importance in relation to the number of times a sample changes its output prediction. 

There is also a large body of active learning work that studies data collection within specific application domains. \cite{logan2022decal} and \cite{logan2022patient} analyze how clinical information can be incorporated into active learning query strategies for the specific dataset in~\cite{prabhushankar2022olives}. \cite{mustafa2021man} utilizes auto-encoder reconstruction information in order to better select samples from seismic volumes. \cite{benkert2022false} introduces the idea of analyzing how out of distribution scenarios manifest in active learning through defining a query strategy with respect to prediction changes during training. Other work \cite{zhang2021deep} has demonstrated the potential of incorporating active learning within multi-modal fusion setups. Although these works are motivated by the practical goal of active learning - to reduce labeling costs, while maintaining a high performance - they each operate on the assumption that annotation costs are constant between instances. The authors in~\cite{settles2008activecost} state that most publicly available datasets are not created with the intention of reducing annotation cost via active learning research. This means that annotation time, or any other form of cost, was not logged for each instance. In their study, they contacted dataset organizers requesting cost data but they were only provided with, "rough estimates about the average annotation time per instance". As such, the authors conducted their own annotation experiments on those datasets to record cost. Before delving more into cost-conscious active learning, we briefly describe how annotation cost has been defined and measured across multiple domains.
\vspace{-2mm}
\paragraph{Cost Measurement} Cost has been defined and measured differently across several domains of cost-conscious active learning. In the domain of natural language processing, \cite{hwa2000sample} proposes to measure cost using the number of brackets within a sentence rather than the number of sentences. Other works use the number of sentences (unit cost) and the number of decisions needed to select a sentence parse (discriminant cost) as metrics to measure cost in active learning \cite{osborne2004ensemble}. In \cite{king2004functional}, the monetary cost of materials used to conduct biological experiments is the bases of quantifying cost. \cite{bloodgood2014bucking} uses annotation time and money as cost metrics. \cite{tomanek2009semi} measures cost by the number of tokens for parts of sentences while \cite{kapoor2007selective} simulates cost to be a linear function of the length of a voicemail message. These are examples of approximate costs being used for active learning. In contrast, \cite{ngai2001rule} measured actual annotation time to compare the efficacy of rule writing versus annotation with active learning. Overall, \cite{baldridge2009well} considered actual annotation time to be the best metric for cost measurement. More recently, \cite{wei2019cost} used lexical and syntactic features to estimate the annotation time of clinical text. 
\vspace{-2mm}
\paragraph{Cost-Conscious Sampling} As it relates to using cost measurements as novel query algorithms in active learning frameworks, \cite{hu2019active} design a query strategy that uses partial labels to reduce cost. \cite{biswas2012active} develop queries with clustering algorithms to remove the need to annotate samples belonging to an already annotated cluster. \cite{qian2013active} and \cite{xiong2015active} both develop similarity-based queries that rank the importance of a sample's neighbors such that less time is needed to label each sample. In \cite{chakraborty2022active}, the authors propose finding a query for temporal data by identifying the optimal subsample size for each queried sample on the task of text classification. They claim their algorithm is generic enough to be used in any domain having temporal data such as video classification. This technique was performed by \cite{vondrick2011video} for video active learning. However, sampling a subset of frames in this manner does not match the human annotation workflow for video data and imposes an impractical method of annotating video data. Also, like many other studies, this method considers cost as constant between samples and only reduces it by querying less frames. 
\vspace{-2mm}
\begin{figure*}[htb!]
\centering
\includegraphics[scale=.40]{Fig/diversity.jpg}
\caption{Examples of Spatial and Temporal Diversity throughout the \texttt{FOCAL} dataset.}
\label{fig: space_temp_diversity}
\end{figure*}
\paragraph{Cost-Available Datasets} We summarize several key characteristics of our FOCAL dataset and other datasets used for cost-conscious active learning in Table \ref{tab:dataset_comparisons}. These works demonstrate how active learning strategies differ based on practical considerations surrounding relevant application settings. The works where approximate cost is reduced by querying fewer samples do not actually represent or reason about cost in practical settings. The studies that use real costs attempt to provide insight on the role of annotation cost in real-world active learning. However, those studies used datasets that did not originally come with annotation cost labels. The authors retrospectively used tools such as Amazon Mechanical Turk to gather the annotations. Retrospective annotations are known to have more sources of confounding error and bias \cite{gerhard2008bias}. \texttt{FOCAL} dataset bridges this gap between simulated and real-world active learning considerations and serves to provide a more robust means of benchmarking active learning algorithms. To the best of our knowledge, \texttt{FOCAL} is the first video dataset intentionally designed for sequential active learning, having real time \textit{prospective cost annotations}. For active learning, this characteristic is crucial as it paves an avenue for cost-oriented active learning approaches that are not exclusively focused on minimizing the amount of annotated data samples. 


==> Sections/Results.tex <==
\begin{figure*}[h!]
\tiny
	\centering
	\includegraphics[width=\textwidth]{Fig/cost_vs_map_compare.png}
	
	\caption{A comparison between cost estimated and probabilistic sampling methods for: (a, d) mAP versus cost. (b, e) cost appreciation rate (CAR) versus cost. (c, f) performance appreciation rate (PAR) versus performance.}
	
	\label{fig:cost-aware-unaware-cpmpare} \vspace{-5mm}
\end{figure*}

\begin{figure}[h!]
\tiny
	\centering
	\includegraphics[width=0.8\columnwidth]{Fig/gflops_analysis.jpg}
	
	\caption{A comparison of overhead cost in Giga-FLOPS (GFLOPS) between inferential and conformal sampling}
	
	\label{fig:gflops} \vspace{-5mm}
\end{figure} 

\section{Results \& Discussion}
\label{sec:results}

\paragraph{Object Detection}
We summarize mean average precision (mAP) at IOU thresholds $0.5$ (mAP@$50$), and mAP between $0.5$ and $0.95$ (mAP@$[50, 95]$) on \texttt{FOCAL} in the last two columns of Table~\ref{tab:detection_benchmarks}. While YOLOv5n has the lowest number of parameters, it achieves the highest test mAP@$50$ around $0.640$. We also show the detection performance of the same architectures on the COCO dataset as mAP@$50$ (COCO). Note that all  models are trained and tested on the $4$ superclasses of \texttt{FOCAL}, while the same architectures are trained on the $80$ object categories of the COCO with higher class complexity. Thus, the overall detection scores of these architectures are lower on the COCO test-dev \cite{redmon2018yolov3, duan2019centernet, Jocher_YOLOv5_by_Ultralytics_2020}. However, \texttt{FOCAL} exhibits various challenges for object detection, especially in the context of infrastructure-based autonomous vehicle research. The challenges include the variation of object size, motion, occlusion, and location, as shown in Fig~\ref{fig: space_temp_diversity}.
Considering the trade-off between performance and training time, we use YOLOv5n in the following active learning experiments.

\input{Tables/ObjectDetectionBenchmarks.tex}

\paragraph{Sequence Active Learning}
The presence of cost labels in \texttt{FOCAL} allows evaluation using mAP versus cost plots, like Figure \ref{fig:cost-aware-unaware-cpmpare}(a, d). We show changes in mAP and cost for 12 rounds of active learning on three unique random seeds in Figure \ref{fig:cost-aware-unaware-cpmpare}(a, d). Shading around each curve represents standard deviation error and the colored dashed vertical lines indicate the total cost of labeling all 13 sampled sequences at the end of 12 rounds. Overall, performance is comparable between both types of sampling methods. However, estimated cost sampling is noticeably cheaper for some strategies. The Min Max Motion sampling (red) in Figure \ref{fig:cost-aware-unaware-cpmpare}(a) has the shortest width overall, indicating it minimizes cost the most while maintaining comparable mAP to all other strategies. Additionally, these plots show more separation between the curves when compared to plots like Figure \ref{fig:intro-cost-perf}(a) that show mAP versus samples. These separations are even more pronounced on CAR and PAR plots. 

We visualize CAR and PAR metrics in Figures \ref{fig:cost-aware-unaware-cpmpare}(b-c, e-f) given budgets in cumulative cost or performance. Specifically, comparing Figures \ref{fig:cost-aware-unaware-cpmpare}(c,f), we see Min Max Motion (red), having the highest CAR overall. This means it is the best at maximizing performance on \texttt{FOCAL} given cost-focused budgets. Conversely, comparing Figures \ref{fig:cost-aware-unaware-cpmpare}(c,f) shows that at a budget of 0.525 mAP, Min Max Motion sampling (red) is the cheapest algorithm overall. However, when the budget is 0.6 mAP Entropy (grey) becomes the cheapest. This stems from the non-linear fashion in which models learn in machine learning. These kinds of analysis are only possible on \texttt{FOCAL} dataset because of the availability of cost labels.   

In Figure \ref{fig:gflops} we show the overhead cost on all available \texttt{FOCAL} data when used for active learning. For inference on a single \texttt{FOCAL} frame, YOLOv5n executes 4.1 GFLOPS. Inference with PWC-Net on a pair of frames to generate an optical flow map utilizes 30.54 GFLOPS. There are $86$ sequences ($76,242$ frames) available for training. The overhead cost of inferential sampling at a single round is the product of 4.1 GFLOPS and the frame count of the remaining sequences in the unlabeled pool at that round. This is computed for each active learning round and then cumulatively summed to arrive at the total overhead cost. Conversely, the total overhead for conformal sampling is the product of 30.54 GFLOPS and the total frames available for training which results in just over 2.3 million GFLOPS. Red shading shows how overhead for inferential sampling cumulatively increases within the theoretical bounds while it remains constant (blue line) for conformal sampling methods. The reason for this is conformal sampling does not do inference on the unlabeled pool at the end of every round. Rather its overhead to compute the flow maps is front loaded and only performed once. The upper and lower theoretical bounds are calculated by selecting sequences in ascending and descending sequence length order respectively, multiplying by 4.1 GFLOPS, then cumulatively summed for all rounds. \vspace{-2mm}


==> Sections/SequenceBM.tex <==
\section{Sequential Active Learning}
With the fine-grained annotation detail and cost information, there is potential for a wide variety of different active learning applications. Due to the high practical relevance, this paper considers both singular, as well as sequential active learning approaches. While the content of this paper is limited to these active learning applications exclusively, we acknowledge that a plethora of other applications are possible and intended.

%\subsection{Definitions}
In batch active learning, the target is to improve data annotation efficiency by involving the model in the selection process. For singular approaches, the active learning algorithm selects the next set of $b$ data samples $X^* = \{x^*_1, ..., x^*_b\}$ from the unlabeled data pool $D_{pool}$ by maximizing an acquisition function $a$:

\begin{equation}
\label{eq:aquisition-function}
    X^* = \argmax_{x_1, ..., x_b \in D_{pool}} a(x_1, ..., x_b | f_w(x))
\end{equation}

Equation~\ref{eq:aquisition-function}, optimizes the number of \emph{single} samples added to $D_{pool)}$ by evaluating the acquisition function on the single samples directly. In literature, this approach is paramount and within this paper we refer to the paradigm as \emph{singular active learning}.

In contrast, the sequential active learning paradigm evaluates the acquisition functions on entire sequences of statistically dependent data in the form of $s_i = \{x_{i,1}, ..., x_{i,N}\}$. Here $x_{i,k}$ represent the individual statistically dependent data points and $N$ the sequence length. Instead of querying individual data samples directly, the acquisition function is adjusted to score individual sequences. Mathematically, this amounts to

\begin{equation}
\label{eq:seq-al}
    S^* = \argmax_{s_1, ..., s_b \in S_{pool}} a(s_1, ..., s_b | g(f_w, s))
\end{equation}

where $g$ represents a summary function that combines the network output of entire data sequences, $S_{pool}$ the unlabeled data sequences. We refer to this approach as \emph{sequential active learning}. In contrast to the singular setting, sequential approaches allow more cost efficient labeling if the samples within a sequence share enough dependencies.

As a final note, we recognize that sequential approaches require an additional definition of a summary function $g$. In our implementations (and \texttt{FOCAL} benchmarks), we reduce $g$ to the arithmetic mean of the individual singular acquisition function values. We acknowledge that different choices are possible and encouraged for future research.




==> Sections/additionalcostanalysis.tex <==
\subsection{Cost Analysis with Modern Annotation Optimizations}
\label{sec:appendix-cost-analysis}
In our cost analysis, we simulate modern annotation software for sequential approaches. Specifically, we estimate singular cost under the assumption of label interpolation and perform experiments with different interpolation rates. We show an example of label interpolation with ten frames of the same FOCAL sequence in Figure~\ref{fig:interpolation-toy}. Instead of annotating every single frame, temporal dependencies can be utilized to interpolate object labels in between two fully annotated frames at nearly zero cost. While static objects result in a simple label copy, dynamic object labels are interpolated through linear mappings as shown in the bottom half of the figure. In this example, we are assuming an interpolation rate of ten - i.e. only every tenth frame is fully annotated. Since the interpolation rate is not static in practical scenarios, we only consider conservative interpolation rates (five, two, and no interpolation).
% Add details about explicit implementations of different strategies here.
\begin{figure}[h]
	\centering
	\includegraphics[width = \columnwidth]{Fig/interpolation-toy.png}
	
	\caption{Label interpolation on a FOCAL sequence. Instead of annotating all objects in every frame, the annotator annotates Frame~1 and Frame~10 and interpolates the remaining labels. For interpolation, a simple linear mapping is used (bottom half).}
	
	\label{fig:interpolation-toy}
\end{figure}

We use the same experimental setup as in the main paper. In order to derive the cost of annotating single frames, we divide the total sequence cost by the effectively annotated frames assuming a fixed frame interpolation rate. For instance, a sequence of 100 sequentially correlated frames can be fully labeled by annotating every 10th frame in detail and interpolating the remaining frames with zero cost. Assuming the entire sequence took 10h to label, the cost-per-frame would be 1h (10h / 10 effective frames). We show the cost in hours for entropy sampling, margin sampling, and least confidence sampling with two, and five respectively (Figure~\ref{fig:cost-single-seq}). For a fair comparison, we additionally include our results with no interpolation that are discussed in the main paper. Complimentary to our previous observations, sequential approaches consistently outperform singular strategies regardless of the interpolation rate.
\begin{figure*}[t]
\centering
\includegraphics[scale=0.45]{Fig/cost-single-seq.png}

\caption{Cost of sequential and single frame entropy sampling, margin sampling, and least confidence sampling on the FOCAL dataset when assuming different interpolation rates. Left: no interpolation. Middle: every second frame in sequence is annotated (rest interpolated). Right: every fifth frame in sequence is annotated (rest interpolated).}

\label{fig:cost-single-seq}
\end{figure*}

==> Sections/tmp.tex <==
\paragraph{Sequence-Wise Active Learning}
We show changes in mAP and cost for 12 rounds of cost-aware and cost-unaware active learning in Figure \ref{fig:cost-aware-unaware-cpmpare} (a, d). The x-axis represents the cost, in hours, of labeling the number of sequences in the training pool and the y-axis is the mAP the model achieved on the test set. Shading around each curve represents standard error and the colored dashed lines indicate the total cost of labeling all 13 sampled sequences at the end of 12 rounds. Overall, performance is comparable between estimated cost sampling and inferential sampling methods, however, estimated cost sampling is noticeably cheaper for some strategies. The Min Max Motion sampling (red) in Figure \ref{fig:cost-aware-unaware-cpmpare}(a) has has the shortest width overall, indicating it minimizes cost the most with comparable mAP to all other strategies. 
% We use the mAP vs cost curves as the basis for all other metrics.

We show visualizations of CAR and PAR metrics in Figures \ref{fig:cost-aware-unaware-cpmpare}(b-c, e-f) given a budget in cumulative cost or performance. Specifically, Figures \ref{fig:cost-aware-unaware-cpmpare}(b,e) answer the question, "With budgets leading up to 200 hours maximum, which algorithm results in the highest performance at each budget?". Here, high CAR values indicate the better algorithm. We see that Min Max Motion sampling (red), having the highest CAR overall at every cost budget, is the best at maximizing performance given a cost-focused budget on \texttt{FOCAL} between estimated cost and inferential sampling algorithms. Conversely, Figures \ref{fig:cost-aware-unaware-cpmpare}(c,f) answer the question, "With budgets leading up to 0.6 mAP, which algorithm achieves the lowest cost at each budget?". Here low PAR values indicate the better algorithm. At each performance budget we see the algorithm best at minimizing cost. For example, at a budget of 0.525 mAP Min Max Motion sampling (red) is the cheapest algorithm overall. However, when the budget is 0.6 mAP Entropy (grey) becomes the cheapest. This stems from the non-linear fashion in which models learn in machine learning. 

These kinds of analysis are only possible on the \texttt{FOCAL} dataset because of the cost labels being present. 



% For our study on cost-unaware methods, we plot performance in mean-average-precision (mAP) versus cost in hours (Figure~\ref{fig:cost-unaware}) and compare the methods entropy \cite{wang2014new}, least confidence \cite{wang2014new}, and FALSE \cite{benkert2022false} to the random baseline. Overall, we observe no clear trends on the cost spectrum. For instance, the strategies least confidence and entropy exhibit significantly different maximum cost values while showing similar mAP values. This is especially surprising as both methods are based on similar softmax statistics and show a similar mAP trend with respect to the number of samples (Figure~\ref{fig:cost-unaware-map}). Further, cost-unaware methods are stochastic in the sequence selection and result in stochasticity both on the cost, as well as the detection performance spectrum. This is especially apparent in Figure~\ref{fig:cost-unaware-map} and \ref{fig:cost-unaware-cost} where we plot video sequences versus mAP and cost separately. In contrast, cost-aware methods are deterministic and result in stochasticity only on the detection performance spectrum (due to e.g. initialization). Finally, we observe that FALSE underperforms the remaining methods in terms of annotation cost; in particular the random baseline. We reason that switch scores vary significantly in video content and are particularly high in dynamic scenes with high cost. Note that even though high cost sequences are selected, the mAP trend of FALSE is competitive with the other methods indicating a clear cost disadvantage. 
% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Fig/cost-unaware.png}
	
% 	\caption{mAP versus cost in hours for the approaches entropy, least confidence, FALSE, as well as the random baseline. We highlight the maximum cost values for each strategy with dashed vertical lines.}
	
% 	\label{fig:cost-unaware}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Fig/cost-unaware-map.png}
	
% 	\caption{mAP versus video samples for the approaches entropy, least confidence, FALSE, as well as the random baseline.}
	
% 	\label{fig:cost-unaware-map}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\columnwidth]{Fig/cost-unaware-cost.png}
	
% 	\caption{Cost in hours versus video samples for the approaches entropy, least confidence, FALSE, as well as the random baseline.}
	
% 	\label{fig:cost-unaware-cost}
% \end{figure}

==> Sections_Kiran_Edits/abstract_v2.tex <==
In this paper, we introduce the \texttt{FOCAL} (Ford-OLIVES Collaboration on Active Learning) dataset which enables the study of the impact of annotation-cost within a video active learning setting. Annotation-cost refers to the time it takes an annotator to label and quality-assure a given video sequence. A practical motivation for active learning research is to minimize annotation-cost by selectively labeling informative samples that will maximize performance within a given budget constraint. However, previous work in video active learning lacks real-time annotation labels for accurately assessing cost minimization and instead operates under the assumption that annotation-cost scales linearly with the amount of data to annotate. \texttt{FOCAL} addresses this discrepancy by providing real annotation-cost labels for 126 video sequences across 69 unique city
scenes with a variety of weather,
lighting, and seasonal conditions. We show through a statistical analysis of the \texttt{FOCAL} dataset that cost is more correlated with the complexity of interactions in a video sequence, rather than its length. We also introduce a set of conformal active learning algorithms that take advantage of these video statistics in order to achieve a better trade-off between annotation-cost and performance while also reducing floating point operations (FLOPS) overhead by at least 77.67\%. We further demonstrate the advantage of these approaches by introducing two performance-cost metrics and show that the best conformal active learning method is cheaper than the best traditional active learning method by 113 hours.  

==> Sections_Kiran_Edits/introduction_v2.tex <==
\section{Introduction}

\begin{figure}[htb!]
\centering
\includegraphics[scale=.35]{Fig/kiran_edit_figures/sequence_length_cost.jpg}
\caption{This shows a plot of the cost vs. sequence length for every video in the \texttt{FOCAL} dataset. The pearson correlation coeffcient between these variables is .21.}
\label{fig: sequence_length_cost}
\end{figure}




\begin{figure}[htb!]
\centering
\includegraphics[scale=.25]{Fig/front_image.jpg}
\caption{This toy example demonstrates the potential trade-off that exists between cost and performance. Two query strategies can potentially select sequences that result in similarly performing models, but have drastically different labeling costs.}
\label{fig: toy_cost_performance}
\end{figure}


\begin{figure*}[htb!]
\centering
\includegraphics[scale=.35]{Fig/kiran_edit_figures/real_world_labeling_active_learning.jpg}
\caption{1) This shows how traditional active learning algorithms processes sequences. All frames of a sequence are equally likely to be selected and labels can be extracted from an Oracle. 2) This shows how in a real world context, annotators are assigned sequences to select to label and then use assistive labeling tools to interpolate between fully labeled frames. This results in both a fully labeled sequence and an associated cost for the work done.}
\label{fig: real_trad_AL}
\end{figure*}


Machine learning has demonstrated the capability to have a major impact in a variety of application areas such as health-care \cite{kokilepersaud2023clinically}, seismology \cite{alaudah2019machine}, and autonomous driving \cite{kokilepersaud2023exploiting}. Despite the potential that machine learning presents, the efficacy of these algorithms is dependent on access to an abundance of high quality labeled data related to the application of interest. This dependence introduces a host of issues because annotating data is an expensive \cite{roh2019survey} and time-consuming process \cite{fredriksson2020data}. This problem is especially prevalent in domains that involve videos \cite{jiao2021new} where long sequences of spatio-temporally correlated frames complicate labeling from both a cost and complexity point of view. Active learning \cite{settles2009active} presents one direction to alleviate these issues due to its ability to reduce annotation-cost by selectively labeling informative samples via a query strategy to maximize performance within a given budget constraint. However, active learning generally and from the perspective of the video domain suffers from two main issues: 1) they make naive assumptions regarding annotation-cost and 2) the framework  of traditional algorithms does not reflect the video annotation process in real-world big data settings.

With regards to point 1, we define annotation-cost as the amount of time it takes an annotator to label and quality-assure their assigned labeling task. Traditional active learning algorithms do not have access to the exact annotation-cost when benchmarking their algorithms and make the assumption that cost shares a linear relationship with the number of samples to be labeled \cite{settles2008activecost}. However, this assumption of a linear
relationship between cost and samples is not valid across
all application domains which includes video. We show in Figure \ref{fig: sequence_length_cost} a plot between annotation-cost of a video and its associated number of frames and demonstrate only a minor correlation with a Pearson correlation coefficient of .21. A variety of other factors beyond just the amount of data can affect annotation-cost which includes motion, object density, occlusion severity, distance of objects
from the sensor, weather, and lighting conditions. The significance of this problem of inaccurate cost estimation can be understood through the toy example of Figure \ref{fig: toy_cost_performance}. In this example, we assume that two active learning strategies select sequences from an unlabeled data pool. Both strategies result in similarly performing models, but the annotation-cost of the sequences selected from query strategy A significantly deviates from that of query strategy B. This highlights the need for active learning algorithms to be benchmarked according to both the annotation-cost and performance of their queried samples. 

The other issue is that the frameworks of traditional active learning strategies do not match how video data is annotated in practice. Many query strategies such as \cite{wang2014new,ash2019deep,benkert2022gauss} were designed on classification tasks that do not take into account spatio-temporal relationships that exist in data. This is shown in part 1) of Figure \ref{fig: real_trad_AL} where the sequence pool $S$ is decomposed to a set of frames from which a query strategy can sample from. This is then labeled by an oracle that provides the labels for the selected data. However, in real world practice annotators are not assigned individual frames, but entire sequences as an annotation task. This is because annotators typically label sequential
frames in blocks \cite{yuen2009labelme}, This is enabled by assistive labeling technology \cite{ashktorab2021ai} that reduces annotator burden by interpolating labels across correlated frames in a video sequence to produce a fully labeled sequence in an efficient manner. All of this is demonstrated by the process shown in part 2) of Figure \ref{fig: real_trad_AL} which results in a labeled sequence with an associated annotation-cost from the time spent by the worker. This discrepancy between real-world practice and standard frameworks suggest that active learning algorithms should be tested in settings that reflect actual annotator practice and that query strategies should be designed that reflect characteristics of the sequential structure of the video domain.

\input{Tables/DatasetComparisons.tex}
In this paper, we address both of these issues of conventional active learning through the introduction of the \texttt{FOCAL} dataset. This is the first video active learning dataset with associated annotation-cost labels for each sequence that was recorded during the labeling of the dataset. Through this dataset, we benchmark active learning algorithms with respect to performance and the cost associated with the queried sequences of each algorithm. Additionally, through an analysis of the dataset we identify factors that contribute to annotation-cost and use these factors to design conformal query strategies. Conformal refers to algorithms that "conform" or make use of the data structure to devise importance scores for sampling. These strategies take advantage of temporal and spatial statistics of video to minimize cost while maximizing performance. We also introduce two new metrics that reflect the interaction between cost and performance. This is done within an active learning experimental setting that reflects real world annotation workflows where entire sequences are selected rather than individual frames. In summary, the contributions of this paper are as follows:

\begin{itemize}
\item We introduce the first public video active learning dataset accompanied by detailed annotations and annotation time, that provides a rigorous basis for accurate quantitative evaluation of annotation cost reduction in active learning research. 
\item We conduct a detailed analysis of multiple factors that affect the annotation cost of video sequences. 
\item We provide a new benchmark for object detection and cost-conscious video active learning on \texttt{FOCAL}. 
\item We compare adaptions of traditional inferential sampling to conformal sampling on video sequences.
\item We introduce two new performance-cost metrics for validating the effectiveness of query strategies minimizing cost while maximizing performance.
\item The presence of video statistics allows us to front-load ranking of the unlabeled pool, thus reducing overhead cost by greater than 8 million GFLOPS.
\end{itemize}


==> Sections_Kiran_Edits/related_works.tex <==

\section{Related Works}


% ------ Outline --------
% Active learning
% Cost measurment
% Cost focused sampling
    %  NLP 
    % video 
% AL for text/video 

%In order to highlight the utility of the \texttt{FOCAL} dataset, an understanding of the gaps in active learning research is necessary. 
%In this section, we first present conventional active learning research, before discussing active learning studies that have more complex problem settings and require extensions to the traditional approaches.

\subsection{Active Learning} Traditional active learning methods typically involve a model iteratively selecting informative samples for annotation from an unlabeled data pool until an annotation budget is reached. Approaches for selecting samples differ in their definition of information content. For example, several approaches define sample importance using softmax probabilities \cite{wang2014new, roth2006margin} where information content is related to the output logits of the network. Other works focus on constructing the core-set of the unlabeled data pool \cite{sener2017active, longtailcoreset}. Furthermore, there are several approaches that consider the combination of both data representation and generalization difficulty within their definition of information content \cite{ash2019deep, prabhushankar2022introspective, haussmann2020scalable}. \cite{batchbald} integrates both generalization difficulty and data representation by extending \cite{houlsby2011bayesian} to diverse batch acquisitions. Recent work \cite{benkert2022gauss} defined sample importance in relation to the number of times a sample changes its output prediction. 

\begin{figure*}[htb!]
\centering
\includegraphics[scale=.40]{Fig/diversity.jpg}
\caption{Examples of Spatial and Temporal Diversity throughout the \texttt{FOCAL} dataset.}
\label{fig: space_temp_diversity}
\end{figure*}


There is also a large body of active learning work that studies data collection within specific application domains. \cite{logan2022decal} and \cite{logan2022patient} analyze how clinical information can be incorporated into active learning query strategies. \cite{mustafa2021man} utilizes auto-encoder reconstruction information to better select samples from seismic volumes. \cite{benkert2022false} introduces the idea of analyzing how out of distribution scenarios manifest in active learning. Active learning has also been applied within the video domain. \cite{bengar2019temporal} made use of temporal coherence information as a means for querying samples. \cite{rana2022all} identified specific frames to label within a video action detection task. Although these works are motivated by the practical goal of active learning - reduce labeling costs, while maintaining a high performance - they each operate on the assumption that annotation costs are constant between instances. The authors in~\cite{settles2008activecost} state that most publicly available datasets are not created with the intention of reducing annotation cost via active learning research. This means that annotation time, or any other form of cost, was not logged for each instance. Our work bridges the gap through the introduction of a dataset with explicit cost labels within a video setting. Additionally, we use a novel experimental setup that utilizes the realistic sequence-wise acquisition paradigm. 

\subsection{Cost Measurement} Cost is defined and measured differently across several domains of cost-conscious active learning. In the domain of natural language processing, \cite{hwa2000sample} propose to measure cost using the number of brackets within sentences. Other works use the number of sentences and the number of decisions needed to select a sentence parse as metrics to measure cost in active learning \cite{osborne2004ensemble}. In \cite{king2004functional}, the monetary cost of materials used to conduct biological experiments is the bases of quantifying cost. \cite{bloodgood2014bucking} uses annotation time and money as cost metrics. \cite{tomanek2009semi} measures cost by the number of tokens for parts of sentences while \cite{kapoor2007selective} simulates cost to be a linear function of the length of a voicemail message. These are examples of approximate costs being used for active learning. In contrast, \cite{ngai2001rule} measured actual annotation time to compare the efficacy of rule writing versus annotation with active learning. Overall, \cite{baldridge2009well} considered actual annotation time to be the best metric for cost measurement. We are the first to provide these measurements for the video domain by defining cost as the time to annotate and quality assure bounding box labels in a full sequence.

\subsection{Cost-Conscious Sampling} Cost-conscious sampling refers to previous work that attempted to integrate cost into  query strategies. For example, \cite{hu2019active} designed a query strategy that uses partial labels to reduce cost. \cite{biswas2012active} develop queries with clustering algorithms to remove the need to annotate samples belonging to an already annotated cluster. \cite{qian2013active} and \cite{xiong2015active} both develop similarity-based queries that rank the importance of a sample's neighbors such that less time is needed to label each sample. In \cite{chakraborty2022active}, the authors propose finding a query for temporal data by identifying the optimal subsample size for each queried sample on the task of text classification. \cite{vondrick2011video} used a video active learning strategy based on selecting identified frames for a video tracking task. However, sampling a subset of frames in this manner does not match the human annotation workflow for video data and imposes an impractical method of annotating video data. Also, like many other studies, this method considers cost as constant between samples and only reduces it by querying less frames. 


\vspace{-2mm}
\subsection{Cost-Available Datasets} We summarize several key characteristics of our FOCAL dataset and other datasets used for cost-conscious active learning in Table \ref{tab:dataset_comparisons}. These works demonstrate how active learning strategies differ based on practical considerations surrounding relevant application settings. The works where approximate cost is reduced by querying fewer samples do not actually represent or reason about cost in practical settings. The studies that use real costs attempt to provide insight on the role of annotation cost in real-world active learning. However, those studies used datasets that did not originally come with annotation cost labels. The authors retrospectively used tools such as Amazon Mechanical Turk to gather the annotations. Retrospective annotations are known to have more sources of confounding error and bias \cite{gerhard2008bias}. \texttt{FOCAL} dataset bridges this gap between simulated and real-world active learning considerations and serves to provide a more robust means of benchmarking active learning algorithms. To the best of our knowledge, \texttt{FOCAL} is the first video dataset intentionally designed for sequential active learning with real time \textit{prospective cost annotations}. 



==> Tables/compare-aware-unaware.tex <==
% \usepackage{multirow}


\begin{table}
\tiny
\centering
\caption{Bla Bla Bla}
\begin{tabular}{cccc|c} 
\toprule
Query Type                    & Query          & \begin{tabular}[c]{@{}c@{}}Cost\\(Hours)\end{tabular} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Best Overhead\\(GFLOPS)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Worst Overhead\\(GFLOPS)\end{tabular}  \\ 
\hline \midrule 
\multirow{4}{*}{Cost-Unaware} & Random         & 666  & 0                                                                                   & 0                                                                 \\
                              & Entropy        & 598  & \multirow{3}{*}{\rotatebox[origin=c]{45}{10,425,508}}                                                         & \multirow{3}{*}{\rotatebox[origin=c]{45}{15,650,589}}                                       \\
                              & Gauss          & 660  &                                                                                     &                                                                   \\
                              & FALSE          & 644  &                                                                                     &                                                                   \\ 
\midrule
\multirow{5}{*}{Cost-Aware}   & Least Frame    & 583  & \multicolumn{2}{c}{\multirow{5}{*}{\rotatebox[origin=c]{45}{2,328,430}}}                                                                                                          \\
                              & Most Frame     & 734  & \multicolumn{2}{c}{}                                                                                                                                    \\
                              & Min Boxes      & 574  & \multicolumn{2}{c}{}                                                                                                                                    \\
                              & Min Motion     & 521  & \multicolumn{2}{c}{}                                                                                                                                    \\
                              & Min Max Motion & 485  & \multicolumn{2}{c}{}                                                                                                                                    \\
\bottomrule
\end{tabular}
\end{table}
